Multi-style Generative Network for Real-time Transfer

Despite the rapid progress in style transfer, existing approaches using feed-forward generative network for multi-style or arbitrary-style transfer are usually compromised of image quality and model flexibility. We find it is fundamentally difficult to achieve comprehensive style modeling using 1-dimensional style embedding. Motivated by this, we introduce CoMatch Layer that learns to match the second order feature statistics with the target styles. With the CoMatch Layer, we build a Multi-style Generative Network (MSG-Net), which achieves real-time performance. We also employ an specific strategy of upsampled convolution which avoids checkerboard artifacts caused by fractionally-strided convolution. Our method has achieved superior image quality comparing to state-of-the-art approaches. The proposed MSG-Net as a general approach for real-time style transfer is compatible with most existing techniques including content-style interpolation, color-preserving, spatial control and brush stroke size control. MSG-Net is the first to achieve real-time brush-size control in a purely feed-forward manner for style transfer. Our implementations and pre-trained models for Torch, PyTorch and MXNet frameworks will be publicly available.

==> sections/4lvls.tex <==

\begin{figure*}
\centering
\subfloat
{
  \begin{overpic}[width=0.19\linewidth]{figure/4levels/Venice-at-the-morning.jpg}
     \put(75,30){\frame{\includegraphics[width=0.05\linewidth,height=0.05\linewidth]{figure/styles/16style.jpg}} }
  \end{overpic}
}
\subfloat
{
\includegraphics[width=0.19\linewidth]{figure/4levels/venice_1.jpg}
}
\subfloat
{
\includegraphics[width=0.19\linewidth]{figure/4levels/venice_2.jpg}
}
\subfloat
{
\includegraphics[width=0.19\linewidth]{figure/4levels/venice_3.jpg}
}
\subfloat
{
\includegraphics[width=0.19\linewidth]{figure/4levels/venice_all.jpg}
}
\par
\setcounter{subfigure}{0}
\subfloat[targets]
{
  \begin{overpic}[width=0.19\linewidth,height=0.12\linewidth]{figure/4levels/grid_0050.jpg}
     \put(75,43){\frame{\includegraphics[width=0.05\linewidth,height=0.05\linewidth]{figure/content/brown-noise.jpg}}}
  \end{overpic}
}
\subfloat[scale 1]
{
\includegraphics[width=0.19\linewidth]{figure/4levels/grid_1.jpg}
}
\subfloat[scale 2]
{
\includegraphics[width=0.19\linewidth]{figure/4levels/grid_2.jpg}
}
\subfloat[scale 3]
{
\includegraphics[width=0.19\linewidth]{figure/4levels/grid_3.jpg}
}
\subfloat[all scales]
{
\includegraphics[width=0.19\linewidth]{figure/4levels/grid_all.jpg}
}
\caption{Visualizing the effects of multi-scale feature statistics for style transfer (top) and texture synthesis (bottom). 
(First column) Input targets; (Center columns)  Inverted representations at each individual scale; (Last Column) Inverted representation combining the multiple scales.
%The first column is the input targets and the other columns show the reversed representations at different scale respectively (the last column combining the multiple scales). 
We use pre-trained 16-layer VGG as the descriptive network and consider the size of 256$\times$256 as the original scale and reduce the size by dividing $2^{i-1}$ for $i$-th scale. The featuremaps after ReLU at each scale are used.}
\label{fig:4lvls}
\end{figure*}



==> sections/msgn.tex <==

\newcommand{\blocka}[2]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{3$\times$3, #1}\\[-.1em] \text{3$\times$3, #1} \end{array}\right]\)$\times$#2}
}
\newcommand{\blockb}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1, #2}\\[-.1em] \text{3$\times$3, #2}\\[-.1em] \text{1$\times$1, #1}\end{array}\right]\)$\times$#3}
}
\newcommand{\blockub}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1, #1}\\[-.1em] \text{3$\times$3, #1}\\[-.1em] \text{1$\times$1, #2}\end{array}\right]\)$\times$#3}
}
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\centering
\begin{adjustbox}{width=0.6\linewidth, height=0.45\linewidth}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
 \hline
 layer name & output size & MSG-Net \\
 \hline
 Conv1 & 256$\times$256& 7$\times$7,64\\
 \hline
 %CoMatch1 & 256$\times$256 & $C$=64\\
 %\hline
  \multirow{3}{*}{Res1} & \multirow{3}{*}{128$\times$128} 
  & \blockb{128}{32}{1} \\
  & & \\
  & & \\\hline
 %CoMatch2 & 128$\times$128 & $C$=128\\
 %\hline
%   \multirow{3}{*}{Res2} & \multirow{3}{*}{64$\times$64} 
%   & \blockb{256}{64}{1} \\
%   & & \\
%   & & \\\hline
 % CoMatch3 & 64$\times$64 & $C$=256\\
 %\hline
  \multirow{3}{*}{Res2} & \multirow{3}{*}{64$\times$64} 
  & \blockb{512}{128}{1} \\
  & & \\
  & & \\\hline
  CoMatch & 64$\times$64 & $C$=512\\
 \hline
 \multirow{3}{*}{Res3} & \multirow{3}{*}{64$\times$64} 
  & \blockb{512}{128}{6} \\
  & & \\
  & & \\\hline
%  \multirow{3}{*}{Up-Res1} & \multirow{3}{*}{64$\times$64} 
%   & \blockub{64}{256}{1} \\
%   & & \\
%   & & \\\hline
  \multirow{3}{*}{Up-Res1} & \multirow{3}{*}{128$\times$128} 
  & \blockub{32}{128}{1} \\
  & & \\
  & & \\\hline
  \multirow{3}{*}{Up-Res2} & \multirow{3}{*}{256$\times$256} 
  & \blockub{16}{64}{1} \\
  & & \\
  & & \\\hline
  Conv & 256$\times$256& 7$\times$7,3\\
 \hline
\end{tabular}
\end{adjustbox}
\caption{The architecture of 32-layer Multi-style Generative Network (MSG-Net).
}
\label{tab:msg-net}
\end{table}



==> sections/structure.tex <==
\begin{figure*}
\centering
\subfloat[target]
{
\includegraphics[width=0.18\linewidth,height=0.12\linewidth]{figure/textures/26style.jpg}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[white noise]
{
  \begin{overpic}[width=0.18\linewidth,height=0.12\linewidth]{figure/structure/26white.jpg}
     \put(75,42){\frame{\includegraphics[width=0.05\linewidth,height=0.05\linewidth]{figure/structure/white-noise-pic.jpg}}}
  \end{overpic}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[Brown noise]
{
  \begin{overpic}[width=0.18\linewidth,height=0.12\linewidth]{figure/structure/26brown.jpg}
     \put(75,42){\frame{\includegraphics[width=0.05\linewidth,height=0.05\linewidth]{figure/structure/brown_noise.jpg}}}
  \end{overpic}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfloat[structured noise]
{
  \begin{overpic}[width=0.18\linewidth,height=0.12\linewidth]{figure/structure/26structure.jpg}
     \put(75,42){\frame{\includegraphics[width=0.05\linewidth,height=0.05\linewidth]{figure/structure/structure.jpg}}}
  \end{overpic}
}
\caption{The synthesized texture images that are triggered by different type of noises.}
\label{fig:noise}
\end{figure*}


